Improving Attention Mechanism with Query-Value Interaction

Attention mechanism has played critical roles in various state-of-the-art NLP models such as Transformer and BERT. It can be formulated as a ternary function that maps the input queries, keys and values into an output by using a summation of values weighted by the attention weights derived from the interactions between queries and keys. Similar with query-key interactions, there is also inherent relatedness between queries and values, and incorporating query-value interactions has the potential to enhance the output by learning customized values according to the characteristics of queries. However, the query-value interactions are ignored by existing attention methods, which may be not optimal. In this paper, we propose to improve the existing attention mechanism by incorporating query-value interactions. We propose a query-value interaction function which can learn query-aware attention values, and combine them with the original values and attention weights to form the final output. Extensive experiments on four datasets for different tasks show that our approach can consistently improve the performance of many attention-based models by incorporating query-value interactions.

==> data/relatedwork.tex <==

\section{Related Work}\label{sec:RelatedWork}
Attention mechanisms have been extensively studied in various NLP tasks in recent years~\cite{YangLWCWT19}. 
A typical kind of attention mechanism is additive attention~\cite{yang2016han}, where the attention query is usually a vector to help recognize important contexts.
It can be applied to the output representations learned by CNN~\cite{yin2016abcnn}, LSTM~\cite{yang2016han} and even self-attention~\cite{WuWYLHX19}.
For example, Yin et al.~\shortcite{yin2016abcnn} proposed to apply additive attention to the feature maps produced by CNNs to select important words to learn more accurate text representations.
Yang et al.~\shortcite{yang2016han} proposed a hierarchical attention network to select important words and sentences simultaneously to learn informative document representations.
Wu et al.~\shortcite{WuWYLHX19} proposed to combine additive attention mechanism with multi-head self-attention to recognize important words based on their contextual representations.
In these methods, the attention query vectors are global parameters, i.e., shared by all different samples.
There are also several variants of the vanilla additive attention~\cite{ma2017interactive,wu2018improving,WuWAHHX19}.
In these methods, the attention queries are hidden representations of the inputs.
For example, Wu et al.~\shortcite{wu2018improving} proposed to use the embeddings of user and item as the attention queries to select important words and sentences according to user preferences and item properties.
Ma et al.~\shortcite{ma2017interactive} proposed to use interactive attention for aspect-level sentiment classification by using the average of word embeddings in targets and contexts as the attention queries for learning target and context representations.
In all aforementioned methods, the output contextual representations are computed based on the attention values, i.e., the input representation sequence.
However, the interactions between the attention query vector and input values are not considered in these methods, which may be very useful for learning accurate output text representations.

Another kind of attention mechanism is dot-product attention~\cite{vaswani2017attention}, where the query is usually a matrix, which contains a set of query vectors.
A popular variant of dot-product attention is self-attention, where the query, key and value come from the same inputs.
A representative neural architecture based on self-attention is Transformer~\cite{vaswani2017attention}, whose core is multi-head self-attention networks.
It is capable of modeling global contexts without recurrence, which is both effective and efficient as the text feature extractor.
Thus, it is broadly used in various state-of-the-art NLP models.
For example, Devlin et al.~\shortcite{devlin2019bert} proposed a bi-directional language representation model named BERT, which can be pre-trained from unlabeled texts by considering contexts in both directions.
Shaw et al.~\shortcite{shaw2018self} proposed to incorporate the relative positions between sequence elements to explicitly consider the orders of words in self-attention networks.
Another representative variant of dot-product attention is co-attention.
In co-attention networks, the inputs are two representation sequences, and they will provide contexts with each other by modeling their relatedness.
For example, Tay et al.~\shortcite{tay2018multi} proposed to use co-attention to model the interactions between the reviews of users and items to enhance their representations.
In self- and co-attention networks, the queries contain the global contexts of the input sequences.
However, in these methods the interactions between queries and values are also not considered, which may be insufficient.
Different from the methods introduced above, our approach can incorporate the interactions of attention queries and values in a unified framework when forming the output representations. 
Experimental results on four datasets in different tasks and languages verify the effectiveness of modeling the query-value interactions in our approach.
